In-medium static inter-quark potential on high resolution quenched lattices

We re-investigate the interactions between static color sources in a finite temperature gluonic medium using both high resolution isotropic and anisotropic quenched lattice QCD ensembles. The underlying ill-posed inverse problem, related to the extraction of spectral functions, is attacked with a range of different methods, including Bayesian inference, Pad\'e interpolation and model fits. Among the latter we include a tail amended Gaussian ansatz and a HTL-inspired fit ansatz. We reconfirm the presence of a dominant low-lying spectral feature that supports the existence of a potential picture for the in-medium evolution of the static charges at late real times. Using the raw unmodified lattice data, all applicable methods show clear signs of screening of the real-part of the potential. After applying a subtraction procedure featured in a previous study we find however that screening disappears from the extracted potential. Paths towards the resolution of this puzzle are discussed.

==> clip.tex <==
%It should be noted that in the past, staggered actions, such as the HISQ action, used in the above study, have been found to exhibit an artificial phase at strong coupling. It is called stripe phase (S4) (see \cite{Kotov:2021mgp} and also \cite{Cheng:2011ic}). In this unphysical phase chiral symmetry is restored, while color charges remain confined. In order to better understand the unexpected results of a confining potential on HISQ lattices at temperatures, where a chirally restored QGP is expected to exist, the question of such unphysical phases needs to be addressed.
